Energy Attacks on Mobile Devices

All mobile devices are energy-constrained. They use batteries that allows using the device for a limited amount of time. In general, energy attacks on mobile devices are denial of service (DoS) type of attacks. While previous studies have analyzed the energy attacks in servers, no existing work has analyzed the energy attacks on mobile devices. As such, in this paper, we present the first systematic study on how to exploit the energy attacks on smartphones. In particular, we explore energy attacks from the following aspect: hardware components, software resources, and network communications through the design and implementation of concrete malicious apps, and malicious web pages. We quantitatively show how quickly we can drain the battery through each individual attack, as well as their combinations. Finally, we believe energy exploit will be a practical attack vector and mobile users should be aware of this type of attacks.

==> application.tex <==
This is the application of this paper


==> apps.tex <==
Exploits can be developed and delivered as apps or webpages. An exploit can be
delivered in an app via several ways.

\begin{itemize}
  \item An app could include the exploits during its development.
  \item During its lifecycle, an app is regularly updated by its authors. The
  update could contain exploits included in them. One update may contain an
  exploit, or an exploit maybe distributed across many updates thus preventing
  any discovery by code review process or malware scanners.
  \item Configuration of an app maybe used to trigger activation of a code
  segment that includes an energy attack, and a different configuration may
  de-activate the attack.
  \item An app can include the attack initially, which can then be de-activated
  by an update. 
  \item An app shows advertisements, which could include scripts to carry out
  energy attacks. The advertisements maybe shown more frequently to drain the
  battery.
    \item By exploiting security services such as carrying out continuous
  authentication, an app can carry out energy attacks.
  \item 
\end{itemize}

An exploit can be delivered by a web-page as follows:
\begin{itemize}
  \item A web-page may contain java-scripts that carry out energy attacks. 
  These java-scripts could contain infinite loops, or recursive code or even a
  sequence of code using software,network and/or hardware elements to drain the
  battery.
  \item The scripts could be delivered to the page via third-party scripts.
  \item The page would also include applets and/or invoke java runtime.
  \item The web-page may include advertisements that are display advertisements,
  which are displayed in a mandatory manner. The advertisements could also
  conytain scripts that carry out energy attacks.
  \item The web-page may also use ajax or such technologies to asynchronously
  download data or carry out computations for draining battery.
  \item CAPTCHA images of large sizes and/or too many CAPTCHAs could be
  downloaded to the device when only one CAPTCHA image of low resolution could
  be useful.
\end{itemize}

Several other techniques could also be employed for apps or web-pages to deliver
the attacks.




==> design.tex <==
For our experiments we used a Samsung Captivate Glide (SAMSUNG-SGH-I927) smart phone with Android Gingerbread (Android version 2.3.6). The components we tested were: CPU, vibration, camera flash, WiFi download, bluetooth, phone, 4G download, brightness, video playback, GPS, notifications, screen rotation, and taking pictures. \\
We also did a control test for comparison. In each of our tests the screen is wake locked, which means the display will not turn off and the phone will not enter sleep mode. This is necessary so that the operating system does not begin powering down components and give inaccurate readings as to their battery usage. Thereby we also acquire the wake lock for the control test. By using this wake locked control we can see how much energy is consumed by each component compared to the wake lock and that should give us an accurate comparison of which components consume more energy.\\
To test the CPU we made two threads that do matrix multiplication. The matrix multiplication starts with two initial matrices and then continues to multiply the resulting matrix by one of the starting matrices. In our experiments this showed CPU utilization of up to 90\%. \\ 
For the camera flash we have an infinite loop that turns the camera's flash on then off. Many current draining applications leave the light on but in theory it will drain more energy when turned off and on continuously. \\
For our testing of the phone functionality we used an echo number. The advantages of an echo number are: it does not require extra participants to receive a call; it does not disconnect prematurely; and it was never busy when we attempted to connect to it. \\
For our download test we have a statically coded address for an image on the web. This image is constantly downloaded and written to the SD-card. Though we could have skipped over writing to the SD-card it seems that a common application would not download something to discard it and would likely constantly store downloaded data for the application. \\
For testing screen brightness we turned the brightness up to its maximum while in our wake locked state. It is important to note that this test would not be accurate without the wake lock. For this component to drain the battery at the levels we record in our experiment, the display must remain active throughout the entire period. It is also important to note that during our experiments we were unable to turn up the brightness when the battery was low (as defined by the Android API).\\
For video playback we load a video from memory and play it in an infinite loop. As wtih the brightness component, this also requires that the phone stay awake and may not functionally drain the battery from the background.\\
To test the GPS component we enabled a location listener and constantly read the location of the device. This is similar to how a GPS would have to be used with a map application, to maintain a current and accurate location.\\
For testing notifications we constantly opened and closed a notification. Though this test does not focus on any hardware components, notifications are very common in consumer applications and we thought it would be important to show their impact.\\
To test the screen rotation we constantly swapped between landscape and portrait layouts. Though this component was tested through API calls, we believe that it is also a reasonable estimate for how the device would drain power when the device is rotated to change screen orientation.\\
To test the photo capability we used the camera interface, rather than the normal method of calling another application to take care of the actual photography. This gave us more control over what components were being used, allowed us to take pictures rapidly, and allowed us to automate the process.\\
For our tests we chose an increment of five percent of the battery to drain. This increment is small enough that testing could be done during a reasonable period of time, but is hopefully large enough that small fluctuations in battery usage should average out over the draining period. For each test the application allows the tester to select which components to enable for the test. Then, when the start button is pressed, the application starts each individual component. After every component has been started the application records the current time and takes an initial reading of the battery level (reported in percent). The main application then sleeps for two second intervals while the component runs. Each time it wakes, it checks the current battery level. If the difference between the original battery level and the current level is below the threshold of five percent, then the application goes back to sleep, with the components still running in the background. If the threshold has been met then the application records the current time, compares it with the starting time and makes a notification to the tester of the number of minutes the application took to drain to the threshold. For our experiments we tested each component ten times. This allows us to take an average that compensates for some of the fluctuations we may see in each individual test.\\
Our next step was to analyze how difficult each component would be to detect. For this we defined a scale of detectability:
\begin{enumerate}
\item Detectable from a distance
\item Detectable during normal usage
\item Detectable with built-in applications
\item Detectable with third party applications
\item Detectable with access to low level functions or system access
\end{enumerate}
Detectable from a distance means that a component could be detected if the device were, for example, in the user's pocket or purse. Detectable during normal usage includes things like a noticeable change in responsiveness of the device. Detectable with built-in applications means that the device comes standard with some program or monitor that detects high usage of a component. Detectable with third party applications means that a component's usage is easily detectable with applications available through the standard marketplace. Detectable with access to low level functions or system access means that to detect a component the user may have to write a program to read and analyze some measurements, or may have to access system logs to find which component is using significant battery power. \\  
These levels were specifically chosen so that any level could be detected with the levels above it and such that the knowledge and experience required increases with each level. At the first two levels we would expect a component's usage to be detected by almost every Android user. At the third and fourth level there is some minimal knowledge of the device required on the part of the user. The user needs to realize that the battery is being drained more than usual, and needs to know where to look for these applications and how to use them. At the fifth level we would only expect a user to detect the drain if the user has some familiarity with development on the Android platform. At the fifth level a user would likely need to actively monitor battery usage and then need the knowledge and experience necessary to write a new application to detect it, or to access system resources to determine the cause. We decided that this would be the highest level as we do not foresee any component being completely unnoticeable or even requiring hardware access to monitor and detect. Because each level requires more knowledge and experience, we seek only the lowest level for each component. This will give an idea of the very minimum amount of knowledge and skill required to detect the use of a component that has a large impact on the battery.\\
For this part of our testing we used our application to turn on each component but did not set a certain battery level threshold. While each component is running we attempt to detect that the particular component is running either at an abnormal level, or running when there should not be an application using that component ( other than our own). We start by attempting to detect it at level one. If significant usage is detected we stop and record the level at which the usage was detected. If, after a reasonable effort, the usage is not detected, we go up to the next step and again attempt to detect the component's usage.  For the purpose of this research we do not attempt to find which application is using the component, but merely that the component is being used in a way that may drain the battery.\\
Finally we give information on each component that may make use of the component more difficult or preventable. We specifically make note of settings that may need to be on for a component to work. This is closely coupled with the permissions required for an application to make use of each component. Knowing this makes it much easier to detect an application that may have a large impact on battery before it is installed. This information allows users to make a more informed decision about whether an application can use the access rights, that the users gives to it, to drain the battery.


==> discussion.tex <==
The most major limitation of our work is the variation in Android implementation across different devices. Because the implementation can vary for each device these numbers may not hold true on different devices. Though the exact numbers may change, we hypothesize that the relative consumption of each component stays about the same. For example: it is likely that the CPU always consumes more energy than downloading over WiFi. Other implementations may also contain different tools for detecting a component's usage. Our research gives a good idea of how some components may drain battery without the user noticing but it opens doors for a lot of future research. Our application uses some common ways to utilize each component but there may be more efficient ways that allow them to drain the battery even faster. We specifically only detect that the component is being utilized but we leave open the question of attribution. Knowing that the device may be draining battery is useful information but identifying which program has initiated these components may be more useful. On a similar topic, there is the possibility of spreading out the work of draining a battery. It may be possible to make requests over other applications such as to indirectly utilize components. Finally more research is needed on how components act during sleep mode and low energy states. When a phone goes to sleep how can applications wake it up? Does the act of waking up a phone consume significant power? What components can be running during sleep mode? Do these components use less power? When the phone is low on power does it compensate by giving less power to each component? Though our research gives an interesting entry into how the battery can be used and abused, there is plenty of room for more research in this area.


==> existing.tex <==
Even though, we are not aware of any malicious implementation of energy attacks
for smartphones running iOS and Android, we have found apps that may carry out
energy attacks inadvertently or as a side effect of other malicious activities
such as data harvesting or a side effect of suboptimized code. Some of the apps
we have found to be draining energy of a device by operations that are not
needed:

\begin{itemize}
  \item ``Flashlight'' by Quick Switch on iPhone 4S: It acquires GPS, sends the
  location to the website perhaps for  location-specific ads and does
  not release it for sometime. It has been found to drain the battery of the
  phone overnight, if the app is not stopped.
  \item Waze app does not release the ``GPS'' for several minutes even though
  the user has stopped using the app. That leads to battery drainage.
\end{itemize}


==> overview.tex <==
This research serves two basic purposes. First is for analyzing battery for normal usage. With typical applications it is important to know how it may be consuming the battery and if the application has any components running in the background that may continue draining battery, even when the application is not being directly used. The second purpose is to analyze the viability of embedding malicious code in an application to intentionally drain the battery. This would mean that an attacker would be able to deny use of the phone to legitimate users, through applications that could be available in standard application markets.In the paper \emph{An Analysis of Power Consumption in a Smartphone} by Aaron Carroll and Gernot Heiser, they took a look at power consumption in a smartphone from a hardware level. Their work focused on a number of common use cases for a smartphone and how much energy was consumed by each component. In our experiments we seek to analyze the usage of many of the same components from an application level. We also seek to show how power usage could be intentionally abused by an attacker from the application layer.  Our goal in the following experiments is to systematically observe, record and analyze Android battery usage and to analyze how difficult it can be to detect a component draining the battery. The first part of this process was designing an application to use each component and measure the battery usage. This application was largely designed in the research by Matthew Stephen and Isaac Strohl. We modified and refined their application to do our experiments on the battery usage of each component. The first part of our experiments was to run each component and record how quickly it drained the battery. For this the application started a component and then waited until a set percentage of the battery was drained. When the application has finished the draining phase, the application makes a notification which includes the number of minutes the application took to drain the defined amount of battery while running the components in each test. With these trials we then calculated an average battery usage for each component. The next step was to analyze how each component could be detected. To do this we start up the application then go through a step by step process of trying to detect the component usage. The process begins with trying to detect the usage just based on outside observations and goes all the way up to checking system logs to find evidence of the component taxing the battery. Each step in the process involves more knowledge and experience with Android than the previous steps. Thereby we search for the first step where we can detect the component which indicates the least knowledge and experience level necessary to positively identify the component as a large factor in battery usage. Finally we include some details on each component and how it could be disabled or prevented by a user. With this information we can show how a component or set of components could drain the battery while maintaining minimum detectability.
